Decrement Operators in Belief Change

While research on iterated revision is predominant in the field of iterated belief change, the class of iterated contraction operators received more attention in recent years. In this article, we examine a non-prioritized generalisation of iterated contraction. In particular, the class of weak decrement operators is introduced, which are operators that by multiple steps achieve the same as a contraction. Inspired by Darwiche and Pearl's work on iterated revision the subclass of decrement operators is defined. For both, decrement and weak decrement operators, postulates are presented and for each of them a representation theorem in the framework of total preorders is given. Furthermore, we present two sub-types of decrement operators.

==> macros_sauerwald.tex <==
% Macros von Kai Sauerwald
\makeatletter
\newcommand{\ifLatexThree}[2]{\@ifpackageloaded{xparse}{#1}{#2}}
\newcommand{\ifMathSCR}[2]{\@ifpackageloaded{mathrsfs}{#1}{#2}}
\newcommand{\ifMathHyperREF}[2]{\@ifpackageloaded{hyperref}{#1}{#2}}
\makeatother


% general stuff:
\ifLatexThree{%
	% LaTeX3 Version:
	\NewDocumentCommand{\headword}{s o m}{\IfBooleanTF{#1}{#3}{\textbf{#3}}\IfNoValueTF{#2}{\index{#3}}{\index{#2}}}%
}{% "Normal" version:
	\makeatletter
	\def\@headword#1{\textbf{#1}\index{#1}}%
	\def\@@headword#1{#1\index{#1}}%
	\def\headword#1{\@ifstar\@headword{#1}\@@headword{#1}}%
	\makeatother
}

\makeatletter
\@ifundefined{naturals}{\newcommand{\naturals}{\mathbb{N}}}{}
\@ifundefined{ol}{\newcommand{\ol}[1]{\overline{#1}}}{}
\makeatother

%%%%%%% Allows a eqref which can break!
% See: https://tex.stackexchange.com/questions/161511/linebreaking-with-eqref-and-long-tags
\makeatletter
\ifMathHyperREF{%
	\newcommand{\seqref}[1]{\hyperref[{#1}]{\textup{\tagform@split{\getrefnumber{#1}}}}}%
}{%
	\newcommand{\seqref}[1]{\textup{\tagform@split{\getrefnumber{#1}}}}%
}
\newcommand\tagform@split[1]{%
	\begingroup
	\m@th\normalfont(\ignorespaces #1\unskip\@@italiccorr)%
	\endgroup
}
\makeatother

% Textbausteine
\newcommand{\ksIF}{\text{if }}
\newcommand{\ksTHEN}{\text{, then }}
\newcommand{\ksAND}{\text{ and }}
\newcommand{\ksOR}{\text{ or }}

\newcommand{\ksST}{\text{ such that }}

\newcommand{\ksForAll}{\text{ for all }}
\newcommand{\ksOtherwise}{\text{otherwise}}

%\newcommand{\naturals}{\ensuremath{\mathbb{N}}} % defined in marcos_ocfs...
\newcommand{\naturalsP}{\ensuremath{\mathbb{N}^+}}
\newcommand{\naturalsZ}{\ensuremath{\mathbb{N}_0}}

\newcommand{\landauBigO}[1]{\ensuremath{\mathcal{O}(#1)}}

% Standard Logik Stuff
\newcommand{\modelsOf}[1]{\ensuremath{\llbracket #1\rrbracket}}
%\newcommand{\beliefsOf}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\negOf}[1]{{\ensuremath{\neg{#1}}}}
\newcommand{\setOfInterp}{\ensuremath{\mathcal{W}}}
%\newcommand{\minof}[2]{\ensuremath{\min(#1,#2)}}

% epistemic states
\newcommand{\beliefsOf}[1]{\ensuremath{B\left(#1\right)}}
\newcommand{\setOfES}{\ensuremath{\Pi}}
\newcommand{\setAllES}{\ensuremath{\mathcal{E}}}
\newcommand{\ksES}{\ensuremath{\Psi}}

% Propositional Logic
\newcommand{\propLang}{\ensuremath{\mathcal{L}}}

% Conditional Logic
\newcommand{\condLang}{\ensuremath{(\propLang|\propLang)}}
\newcommand{\condDOStr}[2]{\ensuremath{\mathrm{str}(#1,#2)}}

% Dalal's revision operator
\DeclareMathOperator{\dalalDiff}{Diff}

% Forgetting dynamics:
%\newcommand{\fdFO}{\ensuremath{\boxminus}} % Fading out
\newcommand{\fdFO}{\ensuremath{\boxbslash}} % Fading out
\newcommand{\fdFOTickSym}{\ensuremath{\bullet}} % Fading out
\newcommand{\fdFOTick}[1]{\ensuremath{{{#1}^{\fdFOTickSym}}}} % Fading out
\newcommand{\fdFOnTick}[2]{\ensuremath{{{#1}^{#2\fdFOTickSym}}}} % Fading out
\newcommand{\fdFI}{\ensuremath{\boxast}} % Fading in
\newcommand{\fdRM}{\ensuremath{\varoast}} % Remembering
\newcommand{\fdIN}{\ensuremath{\varoplus}} % Introduction
\DeclareMathOperator{\introduced}{intro}
\newcommand{\fdFRS}{\ensuremath{(\fdIN,\fdFOTickSym,\fdRM)}}
\newcommand{\simpForgettingSystem}{\fdFRS} % old name
\newcommand{\ksLayer}[3]{\ensuremath{\mathrm{layer}_{#1}(#2,#3)}} % old name
\DeclareMathOperator{\RelHeight}{hgt}

\newcommand{\fdHistory}{\ensuremath{\leadsto}}
\newcommand{\fdHistoryC}{\ensuremath{\leadsto^*}}

% (Proper) Interval orders
\newcommand{\POIsetOfInterp}{\ensuremath{\mathcal{W}^\pm}}
\newcommand{\poi}{\ensuremath{\preceq}}% Total Preorders
%\newcommand{\tpo}{\ensuremath{\leq}}

% Credibility-Limited Revision/Shielded Contraction
\ifMathSCR{%
	\newcommand{\credible}{\ensuremath{\mathscr{C}}}%
}{%
	\newcommand{\credible}{\ensuremath{\mathcal{C}}}%
}

% Useful stuff to copy:
%\DeclareDocumentCommand{\todo}{o g}{\IfNoValueTF{#1}{\begingroup\color{magenta}TODO: #2\endgroup}{\begingroup\color{magenta}#1 #2\endgroup}}

